Measurement of competing pathways in a shock-induced phase transition in zirconium by femtosecond diffraction

The traditional picture of solid-solid phase transformations assumes an ordered parent phase transforms into an ordered daughter phase via a single unique pathway. Zirconium and its prototypical phase transition from hexagonal close-packed (hcp) to simple hexagonal (hex-3) structure has generated considerable controversy over several decades regarding which mechanism mediates the transformation. However, a lack of in situ measurements over the relevant atomistic timescales has hindered our ability to identify the true pathway. In this study, we exploit femtosecond X-ray diffraction coupled with nanosecond laser compression to give unprecedented insights into the complexities of how materials transform at the lattice level. We observe single-crystal zirconium changing from hcp to a hex-3 structure via not one but three competing pathways simultaneously. Concurrently, we also observe a broad diffuse background underlying the sharp Bragg diffraction during the transition. We corroborate our observation of the diffuse signal with multimillion-atom molecular dynamics simulations using a machine-learned interatomic potential. Our study demonstrates that the traditional mechanistic view of transitions may fail for even an elemental metal and that the mechanisms by which materials transform are far more intricate than generally thought.

==> Paper_Clean.tex <==
%\title{\vspace{-4em}\LARGE Complex dynamics during a shock-induced phase transition in Zr}
%\title{\vspace{-4em}\LARGE Transient complexity in phase transformations under shock compression}
%\title{\vspace{-4em}\LARGE Observation of phase transformation complexity: Zirconium $\alpha$$\rightarrow$$\omega$}
\title{\vspace{-4em}\LARGE Measurement of competing pathways in a shock-induced \\phase transition in zirconium by %\emph{in situ} 
femtosecond diffraction}
%\title{\vspace{-4em}\LARGE Observation of anisotropic disorder in a monotonic metal}
%\title{\vspace{-4em}\LARGE Observation of liquid-crystal-like structure \\in zirconium under shock compression}
\author{Saransh Singh\fnref{label1}\corref{cor}}
\ead{saransh1@llnl.gov}
\author{Martin G. Gorman\fnref{label1}}
\author{Patrick G. Heighway\fnref{label2}}
\author{Joel V. Bernier\fnref{label1}}
\author{\\ David McGonegle \fnref{label2,label3}}
% \author{Richard Briggs \fnref{label1}}
\author{Hae Ja Lee\fnref{label4}}
\author{Bob Nagler\fnref{label4}}
\author{Jon H. Eggert\fnref{label1}}
\author{Raymond F. Smith\fnref{label1}}

\cortext[cor]{Corresponding author}
\fntext[label1]{Lawrence Livermore National Laboratory, Livermore, CA, USA}
\fntext[label2]{Department of Physics, Clarendon Laboratory, University of Oxford, Oxford, UK}
\fntext[label3]{Oxford Centre for High Energy Density Science, Department of Physics, Clarendon Laboratory, University of Oxford, Oxford, UK}
\fntext[label4]{Linac Coherent Light Source, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}
%\linenumbers
\maketitle
% Introduction (~ 250 words)
% \textbf{The traditional picture of solid-solid phase transformations assumes an ordered parent phase transforms to an ordered daughter phase via a single unique pathway. This picture adequately explains many fundamental pressure-induced displacive phase transitions in basic elements like carbon \cite{Yagi1992}, silicon \cite{Pandolfi2022}, copper \cite{Sims2022}, and iron \cite{Hawreliak2006}. Zirconium and its prototypical $\alpha\to\omega$ phase transition have proven to be a fertile testbed for our understanding of phase transitions, having generated considerable controversy over several decades regarding which mechanisms mediate the transformation. Our ability to identify the true mechanisms has in part been hindered by a lack of \textit{in situ} measurements over the relevant atomistic timescales. In this study, we exploit femtosecond X-ray diffraction coupled with nanosecond laser compression to give unprecedented insights into the complexities of how materials transform at the lattice level. We observe single-crystal zirconium transforming from $\alpha$ to $\omega$ via not one, but three competing pathways simultaneously, the third of which has never been detected before. Alongside the ordered $\omega$ phase, we observe a partially disordered state unlike any previously seen in an elemental system, possessing the short-range translational order of a glass, but long-range orientational order akin to that of a crystal. We corroborate our observation of the disordered structure with multimillion-atom molecular dynamics simulations using a machine-learned interatomic potential. Our integrated experimental-computational study lays bare the complex dynamics unfolding in zirconium over nanosecond timescales, demonstrating that the traditional mechanistic view of transitions may fail for even an elemental metal, and that the mechanisms by which materials transform are far more intricate than generally thought.
% }
\noindent
\textbf{The traditional picture of solid-solid phase transformations assumes an ordered parent phase transforms into an ordered daughter phase via a single unique pathway. This picture explains many fundamental pressure-induced displacive phase transitions in basic elements like carbon \cite{Yagi1992}, silicon \cite{Pandolfi2022}, copper \cite{Sims2022}, and iron \cite{Hawreliak2006}. Zirconium and its prototypical phase transition from hexagonal close-packed (hcp) to simple hexagonal structure has generated considerable controversy over several decades regarding which mechanism mediates the transformation. However, a lack of \textit{in situ} measurements over the relevant atomistic timescales has hindered our ability to identify the true mechanism. In this study, we exploit femtosecond X-ray diffraction coupled with nanosecond laser compression to give unprecedented insights into the complexities of how materials transform at the lattice level. We observe single-crystal zirconium changing from hcp to a simple hexagonal structure via not one but three competing pathways simultaneously, the third of which has never been detected before. Concurrently, we also observe a broad diffuse background underlying the sharp Bragg diffraction during the transition. We corroborate our observation of the diffuse signal with multimillion-atom molecular dynamics simulations using a machine-learned interatomic potential.  %We observe, for the first time in an elemental system, a partially disordered state, possessing the short-range translational order of a liquid but a long-range orientational bond order akin to that of a crystal. We corroborate our observation of the disordered structure with multimillion-atom molecular dynamics simulations using a machine-learned interatomic potential. The structure in the basal plane predicted by our simulations has remarkable similarities to the smectic phase of a liquid crystal. 
Our integrated experimental-computational approach lays bare the complex dynamics unfolding in zirconium over nanosecond timescales. Our study demonstrates that the traditional mechanistic view of transitions may fail for even an elemental metal and that the mechanisms by which materials transform are far more intricate than generally thought.
}

\smallskip
\noindent
Solid-solid phase transitions have been an active area of scientific inquiry for the last hundred years \cite{Bridgman1912,Bain1924,Kurdjumow1930,Shoji1931,Wassermann1933,Burgers1934,Nishiyama1934}. The lattice-level restructuring brought on by applying sufficient heat or pressure is conventionally measured using X-ray diffraction techniques, yielding direct interatomic separation and coordination measurements. Ultrabright sources such as X-ray free-electron lasers (XFELs) make it possible to realize such measurements \textit{in situ} in solids dynamically compressed to extreme, planetary-scale pressures over mere nanoseconds. Recent research efforts have focused increasingly on using diffraction to pin down not only the structure of exotic high-pressure phases but the atomistic pathway by which that phase is reached \cite{Yagi1992,Hawreliak2006,Pandolfi2022,Sims2022}. 

The conventional picture of the atomistic pathways is based upon atomic mapping from an ordered parent phase to an ordered daughter phase via lattice strain and atomic shuffles. Each transition pathway is differentiated by the orientation with which it leaves the daughter phase relative to its parent. Thus, by measuring the orientation relationship (OR) between specific crystallographic planes and directions within the parent and daughter phases using diffraction, one can experimentally constrain the atomistic transition mechanism.

Due to the commercial and technological importance of zirconium (Zr), titanium (Ti), and their alloys, the transformation mechanism between the ductile $\alpha-$phase (hcp) and the brittle high-pressure $\omega-$phase (simple hexagonal) has been the subject of intense theoretical and experimental scrutiny \cite{SILCOCK1958481,SARGENT1971,RABINKIN1981,UZ1973,Kutsar1990,Swinburne2016,Song1995,Jyoti1997,jyoti2008,osu1070481734,Trinkle2003,Wenk2013,ADACHI20151,wang2019,ZONG2014a,ZONG2014b,Guan2016,Rawat2017,ZONG2019}. Existing literature suggests that two distinct mechanisms can mediate the $\alpha\to\omega$ phase transition. The majority of shock-compression studies on recovered samples have observed what we will call the variant I OR \cite{Song1995,Jyoti1997,jyoti2008} brought about by the TAO-I mechanism \cite{Trinkle2003}. In contrast, the majority of static-compression and high-pressure torsion studies report variant II \cite{SILCOCK1958481,SARGENT1971,RABINKIN1981,Wenk2013,ADACHI20151,wang2019} arising from the Silcock mechanism \cite{SILCOCK1958481}. However, several studies deviate from this trend \cite{UZ1973,Kutsar1990,Swinburne2016} for reasons that remain unclear. A complete understanding of how transition dynamics of this model phase transition depend upon applied loading conditions thus remains elusive.

In this study, we approach the $\alpha\to\omega$ phase transition from a new direction by combining uniaxial laser-shock compression of high-purity, well-oriented single-crystal Zr with \emph{in-situ} diffraction measurements using a high-brightness femtosecond X-ray free electron laser (XFEL) source. The femtosecond probe duration allows us to produce near-instantaneous snapshots of atoms in the high-pressure shocked state as the material is transforming, revealing lattice-level details of the phase transition mechanism. We observe unprecedented transition complexity from the initial simplicity of our single-crystal targets. Unlike previous experimental studies, we observe multiple ORs simultaneously, indicating that several concurrent $\alpha\to\omega$ mechanisms compete within the same shocked volume. We measure both variant I and II ORs, in addition to a third, previously unreported OR (which we refer to as the variant III OR) that vies with variant II OR for dominance. Furthermore, we observe a broad diffuse signal accompanying the sharp Bragg diffraction transition -- a behavior that has never been seen in an elemental metal before. The strength of the diffuse signal decays with increasing pressure.
%consistent with molecular dynamic (MD) predictions of (\ph{*})\ elastic instabilities which form to relieve shear stress \cite{ZONG2014a}.
%We give a detailed lattice-level description for two of the three ORs in Supplementary Materials.
\begin{figure*}[t!]
\includegraphics[width=1\textwidth]{New_Fig1.pdf}
\caption{\label{fig:Fig_1} 
\textbf{$\vert$ Experimental setup for X-ray diffraction measurements of shock-compressed single-crystal Zr samples.} 
\textbf{a.} The 10 keV, 50 fs output of the LCLS-XFEL probed the shock-compressed Zr and produced an X-ray diffraction signal as recorded on CSPad detectors \cite{Hermann2013}.~Here, the diffraction angle ($2\theta$) increases radially, with azimuthal angle ($\phi$) defined around the Debye-Scherrer cones.~This data provides information on crystal structure, sample density, and microstructural texture, while velocimetry measurements provided information on shock timing and pressure uniformity during the X-ray probe period \cite{Celliers2004}.~The diffraction data shown [10.6 GPa] is consistent with multiple reflections from the compressed $\alpha$ phase (red arrows) and a single intense peak from the $\omega-$phase [cyan arrows] (see also Fig.~\ref{fig:Fig_3}\textbf{a}). \textbf{b.} We present the same diffraction data in polar coordinates. The Debye-Scherrer rings appear as straight lines in this view. We present the $\phi$-averaged lineout in the lower panel, where the green curve represents the detector background. The peaks from the $\alpha$ and $\omega-$phase are shaded with red and cyan colors, respectively. We present an enlarged view of the lower-diffraction-angle region in the inset. The lineout to the right of the inset shows the azimuthal variation of the diffuse signal between the Bragg peaks noted by the dashed vertical lines.}
\end{figure*}
We performed laser-driven shock-compression experiments at the Matter in Extreme Conditions (MEC) endstation of the Linac Coherent Light Source (LCLS) \cite{Nagler2015,brown2017}.~We show a schematic of the experimental setup and target design used at MEC in Fig.~\ref{fig:Fig_1}\textbf{a}.~The target consisted of a plastic ablator and a 40-$\mu$m-thick Zr single crystal with the $[0001]$ direction parallel to the sample normal (shock direction). We used an ultrabright XFEL pulse incident normal to the target to perform volume-integrated X-ray diffraction. The scattered X-rays from the shocked Zr sample were recorded by Cornell-Stanford Pixel Array Detectors (CSPADs) in transmission geometry \cite{Hermann2013}.

% The $\alpha\rightarrow\omega$ phase transition in Zr is expected around 10 GPa \cite{dewaele2016}.
% The pressure range can be divided into three distinct regimes (\ph{*})\ :
% \begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
%     \item \textbf{regime (i)}: low-pressure drive, below the $(\alpha \rightarrow \omega)$ phase transition boundary ($<10$ GPa) \cite{dewaele2016}.
%     \item \textbf{regime (ii)}: intermediate-pressure drive, marginally above the phase transition boundary ($10-12.2$ GPa).
%     \item \textbf{regime (iii)}: high-pressure drive, much higher than the phase transition boundary ($\ge$ 12.3 GPa).
% \end{enumerate}
We performed eight experiments with peak pressures ranging from 5.3 to 21.3 GPa. In Fig.~\ref{fig:Fig_1}\textbf{a}, we show the 2D orthographic view of diffraction data for a shock pressure of 10.6~GPa (marginally above the phase transition pressure). While the Zr sample loses its single crystalline nature when shock-compressed to extreme pressures, it retains a highly oriented microstructure, as seen in the localized intensity around the Debye-Scherrer diffraction rings.

We present the same diffraction data in polar coordinates in Fig. \ref{fig:Fig_1}\textbf{b}. The Debye-Scherrer diffraction rings appear as straight lines in this view. We also show the azimuthally averaged variation in diffraction intensity, which we use to identify the different phases in the compressed volume. The 2D diffraction intensity distribution contains information about the evolution of crystallographic texture from the ambient pressure single crystal $\alpha-$phase to the compressed $\alpha$ and phase transformed $\omega-$phase. This information encodes the deformation and phase transition mechanisms activated in the sample \cite{Wehrenberg2017,Pandolfi2022}.

Upon shock compression to 10.6 GPa, diffraction signals from both the compressed $\alpha$ and $\omega-$phases were observed.~We do not observe any diffraction from the uncompressed material ahead of the shock front due to the highly-oriented nature of the zirconium foil (Fig.\ \ref{fig:SM_CSPAD}). We also observe a diffuse background signal superimposed on top of sharp Bragg peaks. This diffuse signal (marked by dashed lines in the Fig.~\ref{fig:Fig_1}\textbf{b} inset) in the intervening regions between the Bragg peaks is observed to be non-uniform azimuthally, and has an angular period of $60^{\circ}$ indicating a sixfold symmetry. The azimuthally localized diffuse signal reveals itself only in our single-crystal scattering configuration; we do not observe it in our polycrystalline Zr diffraction data (see Fig.~\ref{fig:Poly_Zr}).

   \begin{figure*}[t!]
    \centering
    \includegraphics[width=1\textwidth]{New_Fig2_lowres.pdf}
    \caption{\label{fig:Fig_2}
    \textbf{$\vert$ Evolution of diffraction signal as a function of shock pressure.} The experimentally measured 1D azimuthally averaged (top) and full 2D diffraction signal (middle). The forward model predictions are shown in the bottom panel. \textbf{a.} At 10.6 GPa, the 2D and integrated diffraction signals show a combination of both $\alpha-$ (red filled) and $\omega-$phases (cyan filled). A large diffuse scattering background also accompanies the Bragg diffraction. \textbf{b.} At pressures above the onset of the phase transition [12.3 GPa], the $\{0001\}_{\omega}$ and $\{11\bar{2}1\}_{\omega}$ peaks start to emerge. A reduction in the diffuse background accompanies the emergence of these new peaks (see also Fig.\ \ref{fig:Fig_3}b). \textbf{c.} An increase in shock pressure to 15.2 GPa leads to a further reduction in the phase fraction of the $\alpha-$phase and the diffuse scattering intensity. The new $\omega-$phase peaks observed in \textbf{b.}\ increase in intensity. \textbf{d.} At much higher pressures [18.1 GPa], the diffraction signal is composed almost entirely of the $\omega-$phase, with a small amount of diffraction from the compressed $\alpha-$phase, pointing to near complete conversion of the $\alpha \rightarrow \omega$ phase transition. There is a substantial reduction in the diffuse background signal and further evolution in the azimuthal intensity distribution.}
    \end{figure*}

We show the azimuthally averaged intensity, and the experimentally measured 2D diffraction intensity at four pressures above the $\alpha-\omega$ phase-transition boundary in the top two rows of Fig.~\ref{fig:Fig_2}\textbf{a}-\textbf{d}. We have shaded the peaks originating from the $\alpha-$phase in red and the $\omega-$phase in cyan. The $\alpha-$phase, which dominates the diffraction signal at 10.6 GPa, gradually recedes in intensity with increasing pressure. The diffraction signal at 18.1 GPa is almost exclusively from the high pressure $\omega-$phase. Additionally, there is a steady evolution in the azimuthal distribution of diffraction intensity originating from the $\omega-$phase.

To accurately account for the observed diffraction intensity distribution, we constructed a forward model to calculate the expected diffraction signal from the experimental geometry. This model accounts for X-ray beam energy and direction, detector positions, and crystallographic information about the sample, such as crystal structure, unit cell dimensions on compression, phase volume fraction, and the orientation distribution function (texture) of each phase (see Methods section for details).

We present the results of the forward model calculation in Fig.~\ref{fig:Fig_2}\textbf{a}-\textbf{d} bottom row. At 10.6 GPa [Fig.~\ref{fig:Fig_2}\textbf{a}], the compressed sample comprised $85$\% and 15\% phase fractions of the $\alpha-$ and $\omega-$phases, respectively. The $\omega-$phase generates a single strong ring of peaks at $\sim29^{\circ}$ ($\{10\bar{1}1\}_\omega$). The azimuthal texture in this ring reveals the presence of two distinct ORs -- namely variants I and III -- and is, therefore, consistent with two competing phase transformation mechanisms acting within the same shocked volume of zirconium. At a higher shock pressure of 12.3 GPa, we determined the phase fractions of the $\alpha-$ and $\omega-$phases in the compressed volume to be $40$\% and 60\%, respectively. Furthermore, we observe new $\omega-$phase peaks at this pressure. The azimuthal intensity distribution is consistent with variants I and III and a small volume of variant II ORs. A further increase in shock pressure increases the phase fraction of the $\omega-$phase to virtually $100$\%, together with an increase in the volume fraction of variant II at the expense of variants I and III within the $\omega-$phase. For clarity, only the variant contributions to two reflections are shown. We refer the readers to Fig.~\ref{fig:phase_fraction} for our semi-quantitative method of determining the phase fractions of different phases and relative abundance of the various phase transition ORs.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\columnwidth]{New_Fig3_lowres.pdf}% 
    \caption{\label{fig:Fig_3} 
    \textbf{$\vert$ Competing pathways during the $\alpha \rightarrow \omega$ phase transition.} 
    \textbf{a.} Experimental and modeled diffraction patterns from shock-compressed single-crystal zirconium at 10.6~GPa.
    %Top row shows azimuthally integrated lineouts from 2D diffraction patterns, with scattering contributions from $\alpha$, $\omega$ and disordered material separated by color. The middle row shows complete 2D diffraction patterns in $2\theta-\phi$ space. The bottom row shows forward-model calculations for each pressure.\textbf{a.} Diffraction from Zr shocked to low pressure (10.6~GPa). 
    We modeled the crystallographic texture of the $\omega-$phase as the sum of unimodal distributions centered around the $12$ orientations of the variant I OR and $6$ orientations of the variant III OR. We show a close-up of the lower-$2\theta$ region with diffraction from the $\{10\bar{1}0\}_{\alpha}$ and $\{10\bar{1}1\}_{\omega}$ planes. Contributions to the $\{10\bar{1}1\}_{\omega}$ diffraction from the ORs of variants I and III are azimuthally separated and indicated by the cyan and blue arrows, respectively. 
    %The diffuse, disordered signal is localized azimuthally in regions close to the variant III OR peaks. \textbf{b.} Equivalent data taken at intermediate pressure (12.3~GPa). Note that we clocked this sample by $90^{\circ}$ with respect to the sample in \emph{a}, shifting all the reflections by $30^{\circ}$ in the $\phi$ direction after accounting for the $6-$fold symmetry around the compression direction. We modeled the texture as unimodal distributions centered around $12$ variant I, $3$ variant II, and $6$ variant III orientations, with variant III being dominant. \textbf{c.} Equivalent data taken at high pressure (15.2~GPa) with the same sample clocking and texture as in \emph{b}, but with variant II being dominant. 
    \textbf{b.} Phase fraction of each OR formed within the $\omega-$phase volume showing a strong pressure dependence. The variant III OR is dominant at low pressures but is eventually supplanted by variant II OR.}
    \end{figure}
We present the phase-fraction evolution and the relative abundance of the different phase transition ORs with the $\omega-$phase in Fig.~\ref{fig:Fig_3}. We observe a rapid proliferation of the variant II OR with increasing pressures and a decline in the diffuse background signal. Previous theoretical investigation has shown the relationship between shear stress and the dominant OR \cite{ZONG2019}. We speculate the pressure dependence of the ORs shown in Fig.~\ref{fig:Fig_3}\textbf{b} is consistent with an evolving shear stress environment.

    \begin{figure*}[t!]
    \centering
    \includegraphics[width=1\textwidth]{New_Fig4_lowres.pdf}
    \caption{\label{fig:Fig_4}
    \textbf{$\vert$ Molecular dynamic simulations with machine learning potential.} \textbf{a.} Visualization of a Zr single crystal with initial dimensions of $40\times40\times100$~nm\textsuperscript{3} shock-compressed along [0001] to 14~GPa, with atoms colored according to their local phase (above) and shear stress (below) after 18~ps, performed using \textsc{ovito} \cite{OVITO}. Below is the time evolution of the $\alpha$, $\beta$, $\omega$, and noncrystalline phase fractions (the last group includes both partially disordered nanoclusters and atoms on grain boundaries). The circular inset shows the local arrangement of atoms in a region of phase coexistence, viewed in a plane normal to the shock. \textbf{b.} Synthetic diffraction generated 158~ps into the simulation using 10~keV X-rays. The top panel shows the full diffraction pattern in polar coordinates, with a semitransparent mask added to simulate gaps in the CSPad detectors. The lower panel compares azimuthally averaged lineouts from the simulation (14~GPa) and experiment (15.2~GPa). The right panel shows the azimuthal variation of the simulated diffuse signal centered at $2\theta\sim30^\circ$, with averages taken over the windowed region (red-boxed region). We overlay the azimuthal distribution of the azimuthally localized diffuse signal from the experimental data (shot 93) in blue.}
    \end{figure*}

The azimuthally localized yet diffuse diffraction we observe on every shot above the $\alpha\to\omega$ transition pressure signals the presence of a further complexity during the phase transition. To investigate the origin of this diffuse signal, we performed large-scale classical molecular dynamics (MD) simulations of [0001]-oriented Zr single crystals with initial dimensions of $40\times40\times100$~nm\textsuperscript{3} shocked to 14~GPa using \textsc{LAMMPS} \cite{LAMMPS}. We modeled the interatomic interactions using the machine-learned potential of Zong \textit{et al.}\ \cite{ZONG2019}, which was tailored to model allotropy in Zr at pressures of up to 30~GPa. These simulations allow us to see in microscopic detail the dynamics unfolding in the wake of the shock and to analyze the structure factor of the complex atomistic configuration that results.
    
We show in Fig.~\ref{fig:Fig_4}\textbf{a} a visualization of the computational cell 18~ps into the simulation, with atoms colored according to their local phase (above) and shear stress (below). The shock is led by an elastic precursor, behind which the pressure and shear stress are elevated to 10.0~GPa and 3.5~GPa, respectively, but the crystal retains a strained $\alpha$ structure. Trailing this precursor is a phase transition front that raises the pressure to 14~GPa while relaxing the shear stress to 0.9~GPa, heralding the onset of the $\alpha\to\omega$ transition. The parent $\alpha$ phase first transforms to a short-lived ($\sim$10~ps) intermediate $\beta$ (bcc) phase before taking one of two pathways: the $\beta$ nanograins either promptly transform to the $\omega$ structure via a displacive mechanism~\cite{UZ1973}, or they rapidly amorphize and subsequently reconstitute into an anisotropic yet noncrystalline structure via slower diffusive motion. The resulting clusters of partially disordered atoms form 10\% of the cell by mass and occupy the interstices between the larger $\omega$ grains (which constitute 60\%). Though noncrystalline, the atomistic structure of these nanoclusters shows orientational order (see Fig.~\ref{fig:pair-correlation} for the radial and angular distribution functions of the $\beta$, $\omega$, and the noncrystalline structures) and a structure factor qualitatively similar to that of the $\omega-$phase (see Fig.~\ref{fig:structure_factors} for the structure factors of the $\omega$ and noncrystalline structures).

%In agreement with those of Zong \textit{et al.}\ \cite{Zong2020}, our simulations predict that the $\alpha\to\omega$ transition is mediated by a short-lived $\beta$ (bcc) phase. Coexisting with the dominant $\omega$ phase and residual amounts of $\alpha$ and $\beta$, we observe a matrix of disordered material that makes up the remaining 50\% of the shocked material. Examination of the time history of select nanoclusters reveals that the $\beta$ phase forms the `branch point'. After reaching this state, each local environment transforms to either the $\omega-$phase \emph{or} amorphizes and joins the disordered bulk. Most of this disordered material comprises volumes of noncrystalline Zr with no apparent long-range translational order but with strong long-range orientational order. Unlike a truly amorphous structure -- for which the macroscopic distribution of bond directions is perfectly isotropic -- the disordered Zr is characterized by globally directional bonding.
% We examined the disordered structure in a plane parallel to the shock (Fig.~\ref{fig:Fig_2}\textbf{a} inset) and observed a disrupted version of the original $\alpha$-phase basal planes, wherein each bond aligns with one of three universal directions at $120^\circ$ to each other (see Fig.~\ref{fig:pair-correlation} for full 3D pair-correlation functions). We also examined neighboring atomic planes and observed a very similar structure. However, we observed no correlation between the position of the five and seven-fold coordinated atoms between successive planes. We note the remarkable similarities in the structure of disordered Zr normal to the shock direction to the hexatic phase -- an intermediate state between solid and isotropic liquid encountered during melting in two dimensions \cite{Halperin1978,Nelson1979}. Our simulations suggest that the disordered material is stable for at least 0.16~ns, making it feasible to persist over a \textit{ns}-duration experiment. Its lack of translational and strong orientational order makes it a likely candidate to explain the diffuse but azimuthally localized diffraction we observe experimentally. 

In Fig.~\ref{fig:Fig_4}\textbf{b}, we show synthetic diffraction generated by the phase-transformed region of the simulation cell with 10 keV X-rays. Sharp diffraction peaks attributable to $\omega$ grains with the variant II OR are visible at Bragg angles similar to those measured in the experiment and at identical azimuthal angles. The difference in peak intensities is due to the strong sensitivity of the Bragg condition to the $\omega$ phase's $c/a$ ratio, which at 14~GPa takes values of 0.605 and 0.621 in the experiment and simulation, respectively. In addition to these Bragg peaks, we observe a diffuse diffraction signal centered at $29^\circ$ akin to that seen in the data. Like the experimental signal, this diffuse diffraction is anisotropic and exhibits the same sixfold modulations around the Debye-Scherrer ring. While it is tempting to attribute the diffuse scattering to the partially disordered nanoclusters, the truth is subtler: both the crystalline $\omega-$phase and disordered material contribute to the diffuse signal.
Moreover, their contributions do not decompose additively, suggesting they diffract coherently. The signal in question is diffuse because the active scattering vectors are situated far from the sharp maxima in the aggregate's structure factor; the simulations suggest that we are measuring tenuous interpeak scattering intensity that is usually dwarfed by intense Bragg diffraction in a conventional polycrystal experiment. The MD simulations thus account for the diffuse signal that exists alongside the Bragg peaks observed in shock-compressed single-crystal Zr.

%In Fig.~\ref{fig:Fig_4}\textbf{b}, we show synthetic diffraction generated by the phase-transformed portion of the simulation cell with a 10~keV X-ray beam. Diffraction peaks attributable to $\omega$ grains are visible at Bragg angles similar to those measured in the experiment and at identical azimuthal angles. The difference in peak intensities is due to the strong sensitivity of the Bragg condition to the $\omega$ phase's $c/a$ ratio, which at $\sim14$~GPa takes values of 0.605 and 0.621 in the experiment and simulation, respectively. In addition to the Bragg peaks, we observe a diffuse diffraction signal centered at $29^\circ$ akin to that seen in the data. Like the experimental signal, this diffuse diffraction is anisotropic and exhibits sixfold intensity modulations around the Debye-Scherrer ring. To confirm that the disordered Zr is responsible for the broad diffraction signature seen experimentally, we `additively decomposed' the diffraction into contributions from the dominant $\omega$ and disordered phase fractions. As expected, the $\omega$ phase generates the signal observed at the Bragg peaks, while the disordered material is responsible for the bulk of the broad signal at $29^\circ$. We, therefore, conclude from our MD simulations that the textured-disordered diffraction observed in our femtosecond diffraction experiment signals the presence of a previously unobserved, partially disordered state of the elemental metal Zr.

%\sars{\textcolor{red}{[Paddy, feel free to edit as you see fit]} We considered the presence of small $\omega-$phase crystallites and microstrain as a potential source of this signal. However, the crystallite size required to produce the observed full-width at half-maxima via Scherrer's formula \cite{Patterson1939} is $< 1$nm, while a microstrain required would be larger dictated by the volumetric compression ($V/V_{0}$) due to the shock wave. We discard this possibility for the reasons stated above.}
% Having described the origins and nature of the diffuse signal,  

%The crystallographic texture of the compressed $\alpha-$phase was determined using the forward model to be unimodally distributed around the starting orientation with a full width at half maximum of $2^{\circ}$. The texture of $\omega-$phase is determined to be a sum of normally distributed orientation distributions centered around the unique orientations predicted by a single (or multiple concurrent) phase transitions OR(s).

%Alongside the $\omega$ diffraction peaks, we observe a strong diffuse background signal distributed around a broad ring centered at $2\theta\sim28^\circ$. This signal appears to resemble that of an amorphous phase -- such as a liquid or glass -- until one notices its azimuthal dependence, which reveals clear intensity modulations with a period of $60^\circ$ whose maxima coincide with the locations of the OR variant III peaks.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% DISCUSSION %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The new variant III OR we observe in our experiments has never been observed in quenched $\omega-$Zr captured from recovery experiments. This observation is in contrast to numerous experimental static and dynamic compression studies reporting variant I and variant II ORs \cite{SILCOCK1958481,SARGENT1971,UZ1973,RABINKIN1981,Kutsar1990,Song1995,Jyoti1997,jyoti2008,Wenk2013,ADACHI20151,wang2019}.~In a recovery study of shock and pressure released Zr, a complete conversion to the $\omega-$phase during shock loading resulted in only $0$ to $48\%$ in recovered samples, depending on the thermodynamic release path, with a majority of the high-pressure $\omega-$phase reverting to the ambient $\alpha-$phase \cite{gorman2020}. The lack of any experimental observation of the variant III OR in recovered samples could be related to an OR dependence of the $\omega\rightarrow\alpha$ reversion reaction. Upon pressure release, we hypothesize a complete reversion of the variant III $\omega-$phase orientations to the $\alpha-$phase, but hysteresis for variant I and II orientations. We will test this hypothesis in future experiments.

In our MD simulations, the vast majority (99\%) of the $\omega$ phase assumes the variant II OR, with only trace amounts of variant I present. This prediction contrasts with the multi-mechanism picture painted by the experiment. However, the simulation properties can rationalize this behavior. Using quantum mechanical calculations, Trinkle \emph{et al.} \cite{Trinkle2003} reported variant I OR (via the TAO-I pathway) has the lowest potential energy barrier under hydrostatic conditions. Zong \emph{et al.} \cite{ZONG2019}, in their MD study using the identical interatomic potential as our study, have reported a switch in the $\omega-$phase OR from variant II to variant I upon artificially reducing shear stress in their simulations. In our study, we posit that variant I is made rare by the artificially high-shear-stress environment created in these idealistic simulations, in which a planar shock front propagates through a crystal initially devoid of defects that would otherwise permit pre-transition plasticity. Some plasticity before the phase transition will bring about the low-shear-stress environment that favors variant I OR over variant II. Recent measurements by Singh \emph{et al.} on highly oriented Zr \cite{Singh2023} also supports this physical model. In contrast to other static-compression experiments \cite{SILCOCK1958481,SARGENT1971,RABINKIN1981,Wenk2013,ADACHI20151,wang2019}, the authors in that study observe variant I OR  under static-compression where neon was used as a pressure medium to ensure purely hydrostatic conditions. In addition, we believe the absence of variant III in our simulations results from the interatomic potential's inability to accurately model the energy landscape of Zr along the variant III pathway; as this transformation pathway was undiscovered until now, its configuration space did not form part of the database on which the potential was trained. Exploration of this new pathway via first-principles atomistic simulations is warranted.

Our MD simulations predict a small amount of the intermediate bcc $\beta-$phase in the tens of \textit{ps} timescale. Our forward diffraction model predicts that the $\{220\}_{\beta}$ reflection should be observable in our experiments if the OR between the hcp $\alpha-$phase and the bcc $\beta-$phase is the Burger's OR \cite{Burgers1934}. Although not conclusive, our diffraction data hints at the presence of this intermediate bcc phase. We refer the readers to the supplementary materials Fig.~\ref{fig:s96} and section \ref{sec:bcc} for more details.

% Were we to repeat the simulations with preshock microstructure and a realistic `corrugated' shock front, we expect to observe the more equitable distribution of ORs that we see in the experiment. 

% Immediately behind the phase-transition front, the $\alpha$ phase transforms to the $\beta$ phase via rapid atomic shuffling in the $(0001)_\alpha$ plane [the Burgers mechanism~\cite{Burgers1934}]. Thereafter, the majority of the transient $\beta$ phase decays into the stable $\omega$ phase either via further in-plane shuffling (to produce variant II) or out-of-plane shuffling (variant I). Usikov and Zilbershtein~\cite{UZ1973} first hypothesized such an intermediate $\beta-$phase, whose existence has been reported in dynamic compression experiments of polycrystalline Zr using {\it in-situ} X-ray diffraction \cite{Armstrong2021} on subnanosecond timescales. While we see no indication of an intermediate $\beta-$phase in our \textit{ns}-timescale experiment (see Supp.\ Mat.\ Sec.~\ref{sec:beta} for detailed arguments), we do not necessarily expect to, given that the $\beta$ phase is predicted to dominate for only a few picoseconds, and decay to a prohibitively small mass fraction $(\sim5\%)$. We therefore cannot rule out the presence of a transient $\beta-$phase in the \textit{ps} timescale predicted by the simulations. 

% In a static-compression experiment of highly oriented Zr using supercritical Ne as the pressure medium to ensure purely hydrostatic pressure conditions \cite{Klotz2009}, variant I OR was the only $\omega-$phase orientations present \cite{bernier_private}, in line with theoretical predictions \cite{Trinkle2003}. The loading condition encountered in a planar shock experiment is uniaxial strain. Therefore, we expect significant shear stresses in our study.~These observations point to the critical role of shear stress in determining the phase transition mechanism and, consequently, the observed OR. This conclusion is consistent with the findings from an MD study of the $\alpha\rightarrow\omega$ transition in Zr \cite{ZONG2019}, where pre-stressing the initial Zr sample to maintain low deviatoric stress resulted in the variant I OR.

In summary, the dynamic behavior of the elemental metal Zr under shock compression is far more intricate than previously thought, involving multiple competing phase transition pathways and a partially ordered state in a single \textit{ns} shock volume. While we initially attempted to use the more conventional EAM potential for Zr, only the machine-learned interatomic potential reproduced our experimental observations. Our experiments and analysis highlight the importance of \textit{in situ} measurements on highly oriented crystals in validating our best theoretical models at extreme conditions. While our results focus on zirconium, we expect our results to apply to the transformation dynamics of other material systems at high pressure and temperature.

%Measurements made using \textit{in situ} X-ray diffraction of single crystal targets occur in the same timescale as molecular dynamics simulation and can be directly compared to these simulations.
\vspace{-1em}
\noindent
\bibliographystyle{science}
\bibliography{references}
\medskip
\noindent

\noindent\bf Methods

\footnotesize{
\noindent
\textbf{Target.} \normalfont{A schematic of the experimental setup and target design used at MEC is shown in Fig. \ref{fig:Fig_1}.~The target consisted of a 50-$\mu$m thick polyimide ablator, a 40-$\mu$m-thick Zr [0001] single crystal.~The single crystal Zr samples were supplied by Princeton Scientific Corp. The samples were orientated to with $<$ 1$^{\circ}$ of the [0001] axis. An impurity analysis confirmed $>$99.95\% purity and an ambient-pressure density of 6.52 g/cm$^3$.\\

\noindent
\textbf{Forward model.} ~Given a material system with a known crystal structure, lattice parameters, temperature, and crystallographic orientation distribution function, the forward model computes the expected diffraction signal in $2\theta-\phi$ space. In any diffraction experiment in the transmission geometry and a single sample view, only a single ring of the complete pole figure is observable. Therefore, given an orientation distribution function, the forward model modulates the powder diffraction intensity in the azimuthal direction by the observable pole density for each one of the reflections. Fig.~\ref{fig:FM_alpha} shows the complete pole figures for a unimodal orientation distribution centered around the starting orientation of the $\alpha-$phase. We show similar pole figures for the $\omega-$phase for the three observed ORs in \cref{fig:FM_omega_var1,fig:FM_omega_var2,fig:FM_omega_var3}. The dotted magenta circle shows the observable ring of the complete pole figure for each of the reflections. The computation proceeds by the following steps:
\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]
\item For a given material and reciprocal lattice reflection, compute the powder diffraction intensity. The factors include the volume fraction of the phase, unit cell volume, structure factor, Lorentz-polarization factor, the multiplicity of the reflection, and the Debye-Waller factor.
\item Modulate the powder diffraction intensity in the azimuthal direction by multiplying the magnitude of the pole density around the observable ring.
\item Plot the intensity from the previous step as a pseudo-voigt function in $2\theta$ dimension. The full-width half maxima is a function of $2\theta$ via the Cagliotti parameters \cite{CAGLIOTI1958} and particle size, micro-strain parameters. The Thomas-Cox-Hastings profile function \cite{Thompson1987} gives the mixing factor.
\item Apply the mask in $2\theta-\phi$ derived from the composite CSPAD detector.
\end{enumerate}
We performed all computations relating to the orientation distribution function and pole density using the finite element representation of the Rodrigues space fundamental zone \cite{KUMAR1998,Barton2002}.\\

\noindent
\textbf{Laser compression.} ~The output of the 527-nm drive laser at MEC, temporally shaped into a 15-ns flattop pulse, was focused into a 250-$\mu$m spot on the front of the polyimide. This generated an ablatively-driven shock into the target assembly, which an applied uniaxially load along the c-axis of the Zr crystal.~Shock pressure in the sample is directly proportional to the laser intensity, and, therefore precise control of the on-target energy allowed for precise tuning of the pressure within the Zr sample \cite{brown2017}. We set the X-ray probe time in our experiments to ensure the same shock-compressed Zr volume from shot-to-shot, as determined by the velocimetry measurements (Fig. \ref{fig:VISAR}a).\\

\noindent
\textbf{Molecular dynamics simulations.} ~Large-scale classical molecular dynamics (MD) simulations of dynamically compressed zirconium were performed using the open-source code \textsc{LAMMPS}~\cite{LAMMPS}. Interatomic interactions were modeled using the machine-learned potential developed by Zong \textit{et al.}~\cite{ZONG2019}. This short-range classical potential is trained on a reference energy database generated using \textit{ab initio} MD simulations and nudged elastic band calculations. The database includes atomistic configurations representing the $\alpha$, $\beta$, and $\omega$ phases of Zr -- as well as those found along the high-symmetry transition pathways from $\beta\to\alpha$, $\beta\to\omega$, and $\alpha\to\omega$ -- at pressures of up to 30 GPa. In our estimation, this potential is best suited to treating allotropy in Zr at high pressures.

The crystals we simulate are initially defect-free blocks of $\alpha$-Zr with their [0001] direction aligned with the compression axis, $z$. The crystals are subjected to periodic boundary conditions in the transverse directions, $x$ and $y$, to simulate laterally confining material present behind a uniform, uniaxial shock front. All crystals span at least 40 x 40 nm\textsuperscript{2} in the $x$ and $y$ directions to mitigate finite-size effects that might otherwise influence grain growth. Shock waves were driven into the crystal using a momentum mirror ramped to the final particle velocity $U_P$ over 250~ps. A 1-fs timestep is used throughout.

%While the Zong potential is accurate in the gigapascal-pressure regime of interest, it is also costly compared to standard large-scale MD workhorse potentials, such as those belonging to the embedded atom method (EAM) family. To relax the considerable computational requirements of these multimillion-atom MD simulations, we employ two techniques that allow us to model shock compression while simulating no more atomic trajectories than necessary.

To relax computational costs, we use an iterative scheme whereby the length of the crystal is grown incrementally at a rate that keeps pace with the shock front. At every timestep, there exists a tracer layer at a distance $\delta = U_S^e t_{\text{eq}}$ from the crystal's rear surface, where $U_S^e$ is the speed of the elastic precursor wave, and $t_{\text{eq}}$ is the time required for a pristine block of crystal to thermalize ($\sim1$~ps). When the tracer velocity exceeds $0.5U_P^e$, a new block of Zr of thickness $\delta$ is seamlessly appended to the rear surface; the new material thermalizes for at least time $t_{\text{eq}}$ before the shock front sweeps through it. By comparing simulations carried out under an EAM potential with and without this incremental scheme, we have verified that the stress waves generated by the addition of new material (which cause oscillations in the pressure and shear stress of $\pm1\%$ and $\pm5\%$ of their peak values, respectively) do not substantively change the final thermodynamic state reached by the system. By building the `runway' required by the shockwave iteratively -- rather than constructing the crystal with its ultimate dimensions at the outset -- we avoid needless simulation of ambient material waiting to be compressed and thus double our computational efficiency.

We also set a `cutoff time' after which we isolate a relatively small portion of the crystal far behind the shock front for study, and delete the remainder. Once a sufficiently large volume of phase-transformed Zr has accumulated near the front surface, we find the greatest $z$-coordinate at which the average particle velocity is no less than 95\% of the Hugoniot particle velocity $U_P$, insert at this limit a second momentum mirror co-moving with the first at fixed velocity $U_P$, and remove all atoms beyond the second mirror. The remaining block of Zr, which comprises at least 2 million atoms, evolves under constant-volume boundary conditions until the global phase fractions stabilize.

To partition the crystal into its constituent $\alpha$, $\beta$, $\omega$, and noncrystalline phase fractions, we use the following pipeline [executed in \textsc{OVITO}~\cite{OVITO}]:
\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]
\item Following Zong \textit{et al.}~\cite{ZONG2019,Zong2020}, we first classify the atoms according to their Ackland-Jones parameter (AJP) \cite{AcklandJones2006}. Atoms in the $\omega$ phase take AJP values of 2 or 3, depending on whether they are situated on $\omega$'s graphene-like planes or the basal planes that sandwich them, respectively. For brevity, we refer to atoms classified thus as `graphitic' and `basal,' respectively.
\item Atoms in the $\omega$ phase are identified by analyzing their nearest and next-nearest neighbors' AJP values. We count the number of graphitic and basal atoms ($n_g$ and $n_b$, respectively) with which each central atom is coordinated within a cutoff radius of 3.5~\AA. Within this radius, basal atoms should have two basal neighbors and 12 graphitic neighbors; graphitic atoms should have five graphitic neighbors and six basal neighbors. Basal and graphitic atoms whose coordination numbers $(n_g,n_b)$ take the values $(2,12)$ or $(6,5)$, respectively, are assigned to the $\omega$ phase. We give a tolerance of $\pm1$ when comparing coordination numbers to combat thermal fluctuations.
\item Atoms not assigned to the $\omega$ phase are subsequently classified by adaptive common-neighbor analysis (aCNA). Atoms are assigned to $\alpha$ (hcp), $\beta$ (bcc), or `other' structures. The third classification includes atoms in the bulk partially disordered phase, those found on grain boundaries, and `false negatives' whose local crystalline environment was so strongly perturbed by thermal fluctuations as to be unrecognizable to the AJP or aCNA.
\item Atoms whose assigned phase differs from that of all but no more than one of its nearest neighbors are reassigned to the structure of those neighbors. This corrective step further mitigates misidentifications from thermal noise.
\end{enumerate}
Whenever identifying phases, we use atomic coordinates that have been time-averaged over 200~fs (approximately one oscillation period) to further reduce the number of false negatives incorrectly assigned a noncrystalline structure.

To synthesize diffraction patterns from a set of (identical) atoms, we first calculate the ionic structure factor on the locus of $q$-vectors forming the Ewald sphere using the standard expression
\begin{equation}
    S_i(\textbf{q}) = \sum_{\alpha=1}^N e^{-i \mathbf{q} \cdot \mathbf{r}_\alpha}\ ,
\end{equation}
where the $\{\mathbf{r}_\alpha\}$ are the (instantaneous) coordinates of the $N$ atoms of interest. The raw ionic scattering intensity $\lVert S_i(\mathbf{q})\rVert^2$ is calculated and post-multiplied by atomic-form, Lorentz-polarization, and self-attenuation factors.

}
}

\section*{Data availability}
\noindent
\footnotesize{\normalfont{The data supporting the findings of this study are available from the corresponding authors upon reasonable request.
}
}

\section*{Acknowledgements}
\noindent
\footnotesize{\normalfont{We thank the Linac Coherent Light Source (LCLS) operations staff and the Target  Engineering  Team at  Lawrence  Livermore  National  Laboratory  (LLNL)  for assistance in these experiments. The authors would also like to acknowledge Hongxiang Zong and Graeme J. Ackland for generously sharing their machine learning-derived interatomic potential for Zr and Justin Wark for his helpful suggestions during the writing of this manuscript. The research was supported by the Laboratory Directed Research and Development Program at LLNL (project nos.\ 17-ERD-014 and 21-ERD-032). This work was performed under the auspices of the US Department of Energy by Lawrence Livermore National Laboratory under Contract No.\ DE-AC52-07NA27344 (LLNL-JRNL-XXXXXX).} P.\ G.\ H.\ gratefully acknowledges the support of AWE via the Oxford Centre for High Energy Density Science (OxCHEDS).}

\section*{Author Contributions}
\noindent
\footnotesize{\normalfont{S.S., M.G., P.G.H., D.M., J.B., R.B., J.E., and R.S. were involved in all aspects of the experimental design and analysis. B.N. and H-J.L.  were involved in all aspects of the experimental acquisition of data. The manuscript was written by S.S., M.G., P.G.H., J.E., and R.S.and reviewed by all authors.}}

\section*{Competing Interests}
\noindent
\footnotesize{\normalfont{
\noindent The authors declare no competing interests.
}
}

\clearpage
